Towards Nonlinear Disentanglement in Natural Data with Temporal Sparse Coding

We construct an unsupervised learning model that achieves nonlinear disentanglement of underlying factors of variation in naturalistic videos. Previous work suggests that representations can be disentangled if all but a few factors in the environment stay constant at any point in time. As a result, algorithms proposed for this problem have only been tested on carefully constructed datasets with this exact property, leaving it unclear whether they will transfer to natural scenes. Here we provide evidence that objects in segmented natural movies undergo transitions that are typically small in magnitude with occasional large jumps, which is characteristic of a temporally sparse distribution. We leverage this finding and present SlowVAE, a model for unsupervised representation learning that uses a sparse prior on temporally adjacent observations to disentangle generative factors without any assumptions on the number of changing factors. We provide a proof of identifiability and show that the model reliably learns disentangled representations on several established benchmark datasets, often surpassing the current state-of-the-art. We additionally demonstrate transferability towards video datasets with natural dynamics, Natural Sprites and KITTI Masks, which we contribute as benchmarks for guiding disentanglement research towards more natural data domains.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table_graveyard.tex <==
\begin{comment}
\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrrrrrr}
    \toprule
    Model (Data) &  BetaVAE &  FactorVAE &   MIG & MIG (C) & DCI &  Modularity &  SAP & MCC\\
    \midrule
    $\beta$-VAE (S) & 74.0 (3.0) & 53.5 (4.8) & 4.6 (2.6) & 4.7 (2.6) & 9.2 (2.3) & 85.6 (3.9) & 2.2 (1.6) & 38.6 (2.6)\\
    slowVAE (S) & 83.6 (1.2) & 80.5 (2.8) & 19.9 (6.3) & 20.3 (6.6) & 28.8 (5.6) & 86.9 (4.1) & 7.0 (2.4) & 54.6 (2.0)\\
    slowVAE (S-P) & 79.5 (3.3) & 73.8 (6.2) & 16.2 (5.9) & 16.7 (6.3) & 26.3 (6.0) & \textbf{93.0} (2.8) & 3.4 (1.9) & 52.5 (3.7)\\
    \midrule
    $\beta$-VAE (M) & 78.1 (3.0) & 60.6 (6.0) & 4.6 (1.9) & 4.6 (1.9) & 10.3 (1.8) & 87.8 (2.3) & 2.1 (1.0) & 41.7 (3.4)\\
    slowVAE (M) & 82.6 (2.2) & 76.2 (4.8) & 11.7 (5.0) & 12.0 (5.2) & 18.9 (5.5) & 88.1 (3.6) & 4.4 (2.3) & 52.6 (4.1)\\
    slowVAE (M-P) & 77.0 (3.1) & 70.1 (5.7) & 6.9 (3.4) & 7.2 (3.6) & 17.1 (2.5) & \textbf{90.2} (2.5) & 1.7 (0.8) & 49.7 (2.7)\\
    \midrule
    $\beta$-VAE (L) & 78.7 (2.5) & 60.6 (6.1) & 5.3 (2.5) & 5.5 (2.5) & 10.6 (2.3) & 85.4 (3.5) & 2.1 (1.2) & 43.6 (3.7)\\
    slowVAE (L)  & 80.3 (2.8) & 71.1 (9.6) & 6.5 (3.6) & 6.7 (3.8) & 12.3 (3.0) & 86.0 (2.0) & 2.4 (1.2) & 48.6 (4.8)\\
    slowVAE (L-P)  & \textbf{82.5} (2.5) & \textbf{80.2} (6.3) & \textbf{10.4} (3.8) & \textbf{11.0} (4.0) & \textbf{16.7} (3.4) & \textbf{90.1} (1.3) & \textbf{2.5} (0.6) & \textbf{55.3} (4.0)\\
    \midrule
    %\bottomrule
    $\beta$-VAE (C)  & -- & -- & 2.0 & -- & -- & -- & 42.0 & -- & -- & --\\
    slowVAE (C) & -- & -- & 2.8 & -- & -- & -- & 48.7 & -- & -- & --\\
    slowVAE (C-LR) & -- & -- & \textbf{3.4} & -- & -- & -- & \textbf{50.5} & -- & -- & --\\
    %\bottomrule
    \end{tabular}}
\caption{\textbf{Discrete Natural Sprites.} Median (a.d.) performance levels over $10$ random seeds. Best models in each column are indicated in bold font. On nearly all metrics, considering transitions is beneficial.}
\label{table2:performances_discretenatural}
\end{table}

\noindent\begin{table}
\centering
\begin{tabular}{lrrrrrr}
    \toprule
    Model (Data) &  MIG (C) &  MCC \\
    \midrule
    $\beta$-VAE (C)  & 2.2 (1.5) & 42.6 (4.7)\\
    slowVAE (C) & 3.0 (1.7) & 49.1 (4.0)\\
    slowVAE (C-P) & \textbf{3.5} (1.9) & \textbf{52.0} (3.4)\\
    \bottomrule
\end{tabular}%}
\caption{\textbf{Continuous Natural Sprites}. Mean (std) over $10$ random seeds.. 
%Here, we note the comparatively large standard deviations of the continuous MIG score.
}
\end{table}

\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrrrrrr}
    \toprule
    Model (Data) &  BetaVAE &  FactorVAE &   MIG & MIG (C) & DCI &  Modularity &  SAP & MCC\\
    \midrule
    SlowVAE (S) & \textbf{83.4} & \textbf{79.7} & \textbf{21.7} & \textbf{22.1} & \textbf{29.1} & 85.8 & \textbf{7.9} & 54.2\\
   SlowVAE (S-P) & 79.5 & 73.8 & 16.2 & 16.7 & 26.3 & \textbf{93.0} & 3.4 & 52.5\\
    SlowVAE (S-LR) & 82.5 & 77.1 & 14.4 & 14.5 & 22.4 & 87.1 & 6.2 & 52.2\\
    SlowVAE (S-LR-P) & 82.3 & 75.6 & 13.2 & 13.4 & 26.0 & \textbf{93.0} & 5.1 & \textbf{54.4}\\
    \midrule
    SlowVAE (M) & \textbf{83.3} & \textbf{77.2} & \textbf{11.7} & \textbf{12.0} & 18.8 & 87.9 & 4.6 & \textbf{53.9}\\
    SlowVAE (M-P) & 77.0 & 70.1 & 6.9 & 7.2 & 17.1 & \textbf{90.2} & 1.7 & 49.7\\
    SlowVAE (M-LR) & 82.7 & 76.1 & 11.3 & 11.4 & 19.7 & 87.9 & \textbf{5.2} & 52.5\\
    SlowVAE (M-LR-P) & 82.0 & \textbf{77.2} & 9.4 & 9.7 & \textbf{20.1} & 89.4 & 2.9 & 52.5\\
    \midrule
    SlowVAE (L)  & 80.7 & 72.5 & 5.3 & 5.3 & 11.6 & 86.1 & 2.0 & 47.9\\
    SlowVAE (L-P)  & \textbf{82.5} & \textbf{80.2} & \textbf{10.4} & \textbf{11.0} & \textbf{16.7} & 90.1 & 2.5 & \textbf{55.3}\\
    SlowVAE (L-LR)  & 77.5 & 71.7 & 4.9 & 5.1 & 10.5 & 83.3 & 1.8 & 46.3\\
    SlowVAE (L-LR-P)  & 81.9 & 80.0 & 6.7 & 6.8 & 15.7 & \textbf{92.6} & \textbf{2.6} & 52.2\\
    \midrule
    %\bottomrule
    $\beta$-VAE (C)  & -- & -- & 2.0 & -- & -- & -- & 42.0 & -- & -- & --\\
    SlowVAE (C) & -- & -- & 2.8 & -- & -- & -- & 48.7 & -- & -- & --\\
    SlowVAE (C-LR) & -- & -- & \textbf{3.4} & -- & -- & -- & \textbf{50.5} & -- & -- & --\\
    \bottomrule
    \end{tabular}}
\caption{\textbf{Discrete Natural Sprites.} Mean (s.d.) performance levels over $10$ random seeds. Best models in each column are indicated in bold font. On nearly all metrics, considering transitions is beneficial.}
\label{table1:performances_discretenatural}
\end{table}

\begin{table}
%\parbox{.4\linewidth}{
\centering
\begin{tabular}{lrrrrrr}
    \toprule
    Model (Data) &  MIG (C) &  MCC \\
    \midrule
    SlowVAE (C) & 3.0 (1.7) & 49.1 (4.0)\\
    SlowVAE (C-P) & 4.0 (2.5) & 52.8 (4.3)\\
    SlowVAE (C-LR) & 3.3 (1.6) & 50.2 (2.9)\\
    SlowVAE (C-LR-P) & \textbf{5.2} (2.8) & \textbf{54.1} (5.9)\\
    \bottomrule
\end{tabular}%}
\caption{\textbf{Continuous Natural Sprites}. Mean (s.d.) over $10$ random seeds. Considering transitions is beneficial. Here, we note the comparatively large standard deviations of the continuous MIG score.}
\label{table1:performances_continuousnatural}
%$\beta=8$, $\gamma=10$, $\hat{\lambda}=6$}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[ht]
     \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{llllrrrrrrr}
    \toprule
     transition & $\gamma$ & rate\_prior & data & BetaVAE &  FactorVAE &   MIG & MCC & DCI &  Modularity &  SAP \\
    \midrule
    laplace & 10 & 6 & dSprites (LAP) & 100.0 (0.0) &   97.5 (3.0) &   29.5 (9.3) & 69.8 (2.3) & 65.4 (3.6) &  96.5 (1.6) &  8.1 (3.0) \\
    kl\_prev & 16 & -- & dSprites (LAP) & 64.4 (4.1) & 38.8 (10.3) & 5.2 (2.3) & 45.0 (5.5) & 5.9 (3.9) & 93.5 (1.9) & 1.7 (0.8) \\
    kl\_prev & 10 & -- & dSprites (LAP) & 82.9 (5.4) & 60.8 (12.2) & 5.9 (1.8) & 49.2 (4.3) & 13.6 (5.6) & 92.7 (3.0) & 3.9 (1.7) \\
    kl\_prev & 8 & -- & dSprites (LAP) & 83.6 (2.1) & 61.7 (4.7) & 7.1 (2.8) & 48.6 (3.4) & 13.8 (3.9) & 91.0 (2.2) & 4.3 (1.6) \\
    \midrule
    laplace & 10 & 6 & NS (D) & 100.0 (0.0) &   97.5 (3.0) &   29.5 (9.3) & 69.8 (2.3) & 65.4 (3.6) &  96.5 (1.6) &  8.1 (3.0) \\
    kl\_prev & 16 & -- & NS (D) & 72.7 (2.8) & 49.2 (3.7) & 2.8 (1.2) & 38.3 (3.2) & 6.9 (1.8) & 85.3 (1.8) & 1.2 (0.7) \\
    kl\_prev & 10 & -- & NS (D) & 76.6 (3.6) & 52.0 (4.9) & 3.8 (2.2) & 39.0 (3.9) & 7.3 (1.8) & 87.0 (2.2) & 2.0 (1.0) \\
    kl\_prev & 8 & -- & NS (D) & 76.0 (2.4)  & 50.9 (3.7) & 3.4 (2.0) & 38.9 (3.2) & 6.8 (2.2) & 88.4 (1.9) & 1.6 (1.0) \\
    kl\_prev & 4 & -- & NS (D) & 74.0 (3.0) & 49.0 (3.7) & 2.5 (1.6) & 35.7 (3.5) & 6.1 (2.2) & 86.3 (2.3) & 1.6 (0.9) \\
    kl\_prev & 2 & -- & NS (D) & 73.3 (3.0) & 47.9 (4.9) & 2.4 (1.3) & 36.8 (2.4) & 6.1 (1.9) & 87.7 (2.1) & 1.1 (0.6) \\
    \midrule
    laplace & 10 & 6 & NS (C) & & & & 49.1 (4.0) & & & \\
    kl\_prev & 16 & -- & NS (C) & & & & 34.9 (3.6) & & & \\
    kl\_prev & 10 & -- & NS (C) & & & & 33.5 (1.4) & & & \\
    kl\_prev & 8 & -- & NS (C) & & & & 33.5 (3.4) & & & \\
    kl\_prev & 4 & -- & NS (C) & & & & 33.8 (2.0) & & & \\
    \midrule
    laplace & 10 & 6 & KITTI ($\Delta t=1$) & & & & 66.1 (4.5) & & & \\
    kl\_prev & 16 & -- & KITTI ($\Delta t=1$) & & & & 63.1 (9.3) & & & \\
    kl\_prev & 10 & -- & KITTI ($\Delta t=1$) & & & & 57.4 (8.5) & & & \\
   kl\_prev & 8 & -- & KITTI ($\Delta t=1$) & & & & 59.0 (5.6) & & & \\
   kl\_prev & 4 & -- & KITTI ($\Delta t=1$) & & & & 51.8 (9.2) & & & \\
   kl\_prev & 2 & -- & KITTI ($\Delta t=1$) & & & & 50.3 (7.4) & & & \\
   kl\_prev & 1 & -- & KITTI ($\Delta t=1$) & & & & 38.4 (6.8) & & & \\
    \midrule
    laplace & 10 & 6 & KITTI ($\Delta t=5$) & & & & 79.6 (5.8) & & & \\
    kl\_prev & 16 & -- & KITTI ($\Delta t=5$) & & & & 69.6 (5.9) & & & \\
    kl\_prev & 10 & -- & KITTI ($\Delta t=5$) & & & & 78.2 (6.0) & & & \\
   kl\_prev & 8 & -- & KITTI ($\Delta t=5$) & & & & 73.8 (10.0) & & & \\
   kl\_prev & 4 & -- & KITTI ($\Delta t=5$) & & & & 67.9 (10.4) & & & \\
   kl\_prev & 2 & -- & KITTI ($\Delta t=5$) & & & & 60.7 (8.8) & & & \\
   kl\_prev & 1 & -- & KITTI ($\Delta t=5$) & & & & 60.9 (9.1) & & & \\
    \bottomrule
    \end{tabular}}
     \caption{kl\_prev}
     \label{tabel:all_results_dsprites}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[ht]
     \centering
    %\resizebox{\textwidth}{!}{\begin{tabular}{lr}
    \begin{tabular}{lr}
    \toprule
      $\text{max}(\Delta\text{frames})$ & MCC \\
    \midrule
    1 & 66.1 (4.5) \\
    3 & 76.5 (4.7) \\
    5 & 79.6 (5.8) \\
    7 & 83.2 (3.9) \\
    9 & 85.4 (3.3) \\
    11 & 83.3 (5.6) \\
    13 & 88.6 (3.3) \\
    15 & 87.6 (4.4) \\
    17 & 86.3 (4.4) \\
    19 & 85.7 (6.3) \\
    21 & 87.0 (5.1) \\
    23 & 86.5 (7.4) \\
    25 & 89.2 (1.4) \\
    27 & 85.7 (7.0) \\
    29 & 89.3 (2.4) \\
    33 & 88.4 (3.8) \\
    37 & 87.2 (3.5) \\
    41 & 88.3 (3.7) \\
    45 & 88.6 (2.2) \\
    49 & 88.6 (2.3) \\
    53 & 87.7 (3.0) \\
    57 & 87.6 (3.3) \\
    \bottomrule
    %\end{tabular}}
    \end{tabular}
     \caption{slowvae kitti}
     \label{tabel:all_results_dsprites}
\end{table}
\end{comment}

\begin{comment}
\begin{table}
     \centering
     \begin{tabular}{lrrrrrr}
     \toprule
     Model (Data) &  BetaVAE &  FactorVAE &   MIG &  DCI &  Modularity &  SAP \\
     \midrule
     $\beta$-VAE (\textit{i.i.d.}) & 82.3 & 66.0 & 10.2 & 18.6 & 82.2 & 4.9 \\
     Ada-ML-VAE (LOC) & 89.6 & 70.1 & 11.5 & 29.4 & 89.7 & 3.6 \\
     Ada-GVAE (LOC) & 92.3 & 84.7 & 26.6 & 47.9 & 91.3 & 7.4 \\
     SlowVAE (UNI) & 90.4 (3.3) & 81.35 (7.6) & 35.7 (8.3) & 52.1 (6.5) & 87.6 (2.0) & 5.1 (1.4) \\
     SlowVAE (LAP) & 100.0 (0.0) & 98.32 (2.5) & 27.8 (7.9) & 65.3 (3.1) & 97.0 (1.5) & 6.1 (2.6) \\
     \bottomrule
     \end{tabular}
     \caption{\textbf{DSprites.} Median and absolute deviation (a.d.) metric scores across 10 random seeds (first three rows are from \citep{locatello2020weakly}). Results for additional datasets and metrics are in Appendix~\ref{sec:additional_results}.
     }
     \label{table1:performances_dsprites}
     %\vspace{-15pt}
\end{table}

\begin{wraptable}{R}{.75\textwidth}
    \vspace{-15pt}
     \centering
    \begin{tabular}{lrrrrr}
    \toprule
                      Model (Data) &  SN &  Cars3D &  Shapes3D &  MPI3D \\
    \midrule
                   $\beta$-VAE (\textit{i.i.d.}) &       21.4 &           8.8 &          22.0 &           7.2 \\
     Ada-ML-VAE (UNI) &       31.1 &    14.7 &      50.9 &   24.1 \\
       Ada-GVAE (UNI) &       25.6 &    15.0 &      56.2 &   28.4 \\
           %SlowVAE (UNI) &       24.9 (1.4) &  \textbf{15.5} (1.4) &  \textbf{66.4} (5.9) &  \textbf{37.4} (6.6) \\
           SlowVAE (UNI) &  23.2 (1.9) &  15.5 (1.4) &  66.4 (5.9) &  33.1 (1.2) \\
          %SlowVAE (LAP) &       27.7 (0.7) &   9.8 (1.4) &  62.9 (3.4) &  26.1 (2.9) \\
          SlowVAE (LAP) & 25.4 (0.6) &   9.8 (1.4) &  62.9 (3.4) &  29.6 (1.1) \\
    \bottomrule
    \end{tabular}
     \caption{\textbf{DisLib Benchmarks.} Median (a.d.) MIG scores across 10 random seeds (first three rows are from \citep{locatello2020weakly}). SN refers to SmallNORB.}
     \label{table1:performance_main}
\vspace{-15pt}
\end{wraptable}
\end{comment}
